The Effectiveness of Subsidies and Tolls in Congestion Games

Are rewards or penalties more effective in influencing user behavior? This work compares the effectiveness of subsidies and tolls in incentivizing user behavior in congestion games. The predominantly studied method of influencing user behavior in network routing problems is to institute taxes which alter users' observed costs in a manner that causes their self-interested choices to more closely align with a system-level objective. Another conceivable method to accomplish the same goal is to subsidize the users' actions that are preferable from a system-level perspective. We show that, when users behave similarly and predictably, subsidies offer superior performance guarantees to tolls under similar budgetary constraints; however, in the presence of unknown player heterogeneity, subsidies fail to offer the same robustness as tolls.

==> atomic_congestion_games.tex <==
\section{Atomic Congestion Games}\label{sec:atomic}
The preceding results on subsidies and tolls have been presented in the context of \textit{non-atomic} congestion games, in which the set of infinitesimal users comprise a continuum of players~\cite{Schmeidler1973}.
Though this setting has been prominent in traffic routing problems~\cite{Wardrop1952}, study has also been devoted to the case where there are a finite number of users, known as \textit{atomic} congestion games~\cite{Rosenthal1973}.
In the literature, many of the results in the non-atomic setting do not similarly hold in the atomic; however, several of the results in this manuscript hold for both settings.

To formalize the notation of an atomic congestion game, we use the same model as in \cref{sec:prelim} but replace the definition of a flow $f$.
An atomic flow is a vector $f \in \mathbb{Z}_{\geq 0}^{|\mathcal{P}|}$ that expresses the \textit{number} of users utilizing each path.
The number of users on an edge $e \in E$ is thus $f_e = \sum_{P:e\in \paths} f_P$, and we say $f = \{f_e\}_{e \in E}$.
A flow $f$ is \textit{feasible} if it satisfies $\sum_{P \in \paths_i}f_P = r_i$ for each source-destination pair, where $r_i$ is the number of users traveling from origin $o_i$ to destination $d_i$.
Now, the set of users in the system $N$ is finite and has size $|N| = \sum_{i=1}^k r_i$.

Though the change in the definition of the problem is small, many of the results and intuitions between the two problems differ greatly, particularly in the price of anarchy~\cite{Roughgarden2002,Christodoulou2005},\cite{Bergendorff1997,Bilo2016},\cite{Pigou1920,Paccagnan2019I}.
However, in this work, when comparing the price of anarchy under subsidies and tolls in homogeneous and heterogeneous settings, many of the results and intuitions persist in both settings.

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{"atomic_poa".png}
\caption{\small Price of anarchy of optimal bounded subsidies and tolls in polynomial atomic congestion games with degree $p=4$. Under each incentive bound $\beta$, subsides provide better performance guarantees than tolls as in \cref{thm:bounded}.}
\label{fig:atomic_poa_figure}
\end{figure}

\begin{corollary}
\cref{thm:bounded}, \cref{thm:lim}, and \cref{thm:robust} each hold for atomic congestion games.
\end{corollary}
\emph{Proof Outline:} The proofs for \cref{thm:bounded}, \cref{thm:lim}, and \cref{thm:robust} can each be replicated by replacing $N$ with a countable set and redefining $\ell_e:\mathbb{Z}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ for all $\ell_e \in L(\gee)$, where each players' cost function is defined as before but is now a mapping from non-negative integers.
Each proof uses the same equilibrium condition which does not change in the atomic setting.
Every other argument follows similarly to the non-atomic setting.

From this, the following results remain in the atomic setting: (1) when users are homogeneous in their response to incentives, subsidies provide better performance guarantees with smaller monetary transactions, (2) the performance of subsidies degrades more quickly as users become heterogeneous in their response to incentives, and (3) significantly large tolls can mitigate the effect of user heterogeneity.

To see at least part of this, we can compare the effectiveness of optimal incentives with homogeneous users with methods proposed in~\cite{Paccagnan2019I}.
Let $\gee$ be a family of atomic congestion games and $B = \{b_1,\ldots,b_m\}$ be a set of basis latency functions such that $L(\gee)$ is the set of all linear combinations of elements in $B$.
The optimal incentives and the resulting price of anarchy are both the solution to a tractable linear program.


\begin{theorem}%[Optimal tolls]
\emph{(Paccagnan} \textit{et al.}~\emph{\cite{Paccagnan2019I})} Let $\ell(x)=\sum_{j=1}^m \alpha_j b_j(x)$ be a latency function.
A local incentive mechanism minimizing the price-of-anarchy is given by
	\[
    \opt{T}(\ell) = \sum_{j = 1}^{m} \alpha_j\cdot \opt{\tau}_j,\quad\text{where}\quad \opt{\tau}_j(x) = \opt{f}_{j}(x) - b_j(x),
    \] 
%    \[
%    \opt{T}(\ell) = \sum_{j = 1}^{m} \alpha_j\cdot \opt{T}(b_j),\quad\text{where}\quad \opt{T}(b_j) = \opt{f}_{j} - b_j,
%    \]
    %where 
    % \[ T^*(b_j) = \tau_j^*(|a|_r,\alpha_j) = \alpha_j \left(f_{j}^{\mathrm{OPT}}(|a|_r) - b_j(|a|_r)\right), \]
   % $ \opt{T}(b_j) = \opt{f}_{j} - b_j$
   and $\opt{f}_{j}:\{1,\dots,n\}\rightarrow\mb{R}$ is a solution to the linear program\footnote{Note that each constraint appearing in \eqref{eq:mainLPopt} is obtained for a different choice of the tuple $(x,y,z)$, and is therefore a linear expression of the unknowns $f_j$ and $\rho$. While in this formulations there are $\mc{O}(n^3)$ constraints, these can be reduced to only $\mc{O}(n^2)$, see \SM.}
%\[
\begin{equation}\label{eq:mainLPopt}
\begin{split}
        &\max_{f_j \in \mathbb{R}^n, \rho \in \mathbb{R}}  \rho\quad\text{s.t.}\\
        &
        \hspace{6mm} b_j(x\hspace*{\mynegspace}+\hspace*{\mynegspace}z)(x\hspace*{\mynegspace}+\hspace*{\mynegspace}z)\hspace*{\mynegspace}-\hspace*{\mynegspace}\rho b_j(x\hspace*{\mynegspace}+\hspace*{\mynegspace}y)(x\hspace*{\mynegspace+\hspace*{\mynegspace}y)}\hspace*{\mynegspace}\\
        & \hspace{40mm}+\hspace*{\mynegspace}f_j(x\hspace*{\mynegspace}+\hspace*{\mynegspace}y)y\hspace*{\mynegspace}-\hspace*{\mynegspace}f_j(x\hspace*{\mynegspace}+\hspace*{\mynegspace}y\hspace*{\mynegspace}+\hspace*{\mynegspace}1)z\hspace*{\mynegspace}\ge\hspace*{\mynegspace}0\\
        %b_j(y)y - \rho b_j(x)x + (x-z)f(x) - (y-z)f(x+1) \geq 0 \\
        & \hspace*{28mm}\forall\,(x,y,z) \in \mb{N}^3~\text{with}~1\le x+y+z \le n,\\[1mm]
        &\hspace{6mm}f_j(x)\ge 0 \hspace*{8mm}\forall x\in\{1,\dots,n\},
\end{split}
\end{equation}
where we define $b_j(0)=f_j(0)=f_j(n+1)=0$ to ease the notation.
%where $\IR=\{(x,y,x)\in\mb{N}^3~s.t.1\le x+y-z \le n\}$
The resulting optimal price-of-anarchy is $\max_{j}\{1/\opt{\rho}_j\}$, where $\opt{\rho}_j$ is the value of the linear program in \eqref{eq:mainLPopt}.
%\]
%\DP{$\mc{I}$}\\
%\DP{The optimal price of anarchy is $1/\rho^\star$}.
\end{theorem}

By solving \eqref{eq:mainLPopt}, the price of anarchy under an optimal incentive mechanism can be computed.
Further, the linear program can be modified to include a budgetary constraint as well as limit the search to either subsidies or tolls respectively.
To restrict \eqref{eq:mainLPopt} to solve for the optimal toll with incentive bound $\beta$, an additional decision variable $\nu \geq 0$ is included, as well as the constraints
\begin{align*}
f_j(x) - \nu b_j(x) &\geq 0 ~~ &&\forall x \in \{1,\ldots,n\},\\
f_j(x) - \nu b_j(x) &\leq \nu\beta b_j(x) ~~ &&\forall x \in \{1,\ldots,n\}.
\end{align*}
Similarly, to restrict \eqref{eq:mainLPopt} to solve for the optimal subsidy with incentive bound $\beta$, an additional decision variable $\nu \geq 0$ is included, as well as the constraints
\begin{align*}
f_j(x) - \nu b_j(x) &\leq 0 ~~ &&\forall x \in \{1,\ldots,n\},\\
f_j(x) - \nu b_j(x) &\geq -\nu\beta b_j(x) ~~ &&\forall x \in \{1,\ldots,n\}.
\end{align*}


To illustrate that \cref{thm:bounded} holds for atomic congestion games, consider the class of polynomial congestion games with latency functions of order at most 4, i.e., \mbox{$B = \{1,x,x^2,x^3,x^4\}$}.
In \cref{fig:atomic_poa_figure}, the solution to \eqref{eq:mainLPopt} for this class of congestion games is computed using varying budgetary constraints for tolls and subsidies respectively.
Observe that for similar budgetary constraints, subsidies outperform tolls, as predicted by \cref{thm:bounded}.

Computing optimal incentives in atomic congestion games with user heterogeneity is currently an open area of research, however \cref{thm:lim} and \cref{thm:robust} give insight into how tolls and subsidies compare in performance.


